CSI: Novelty Detection via Contrastive Learning on Distributionally Shifted Instances

Novelty detection, i.e., identifying whether a given sample is drawn from outside the training distribution, is essential for reliable machine learning. To this end, there have been many attempts at learning a representation well-suited for novelty detection and designing a score based on such representation. In this paper, we propose a simple, yet effective method named contrasting shifted instances (CSI), inspired by the recent success on contrastive learning of visual representations. Specifically, in addition to contrasting a given sample with other instances as in conventional contrastive learning methods, our training scheme contrasts the sample with distributionally-shifted augmentations of itself. Based on this, we propose a new detection score that is specific to the proposed training scheme. Our experiments demonstrate the superiority of our method under various novelty detection scenarios, including unlabeled one-class, unlabeled multi-class and labeled multi-class settings, with various image benchmark datasets. Code and pre-trained models are available at https://github.com/alinlab/CSI.

==> resources/tab_rot_align.tex <==
\begin{wraptable}[10]{r}{0.4\textwidth}
\vspace{-0.25in}
\centering\small
~\caption{
AUROC (\%) on DTD dataset, where Textile is used for OOD.
}\label{tab:rot_align}
\vspace{0.04in}
\begin{minipage}{0.095\textwidth}
\includegraphics[width=\textwidth]{figures/woven.jpg}
\end{minipage}
\begin{minipage}{0.095\textwidth}
\includegraphics[width=\textwidth]{figures/chequered.jpg}
\end{minipage}
\begin{minipage}{0.095\textwidth}
\includegraphics[width=\textwidth]{figures/interlaced.jpg}
\end{minipage}
\begin{minipage}{0.095\textwidth}
\includegraphics[width=\textwidth]{figures/spiralled.jpg}
\end{minipage}
%
\begin{minipage}{0.3\textwidth}
\vspace{0.08in}
\centering\small
\begin{tabular}{ccc}
\toprule
Base & CSI (Rotation) \\
\midrule
92.9 & 65.4 \\
\bottomrule
\end{tabular}
\end{minipage}
%
\end{wraptable}
